Differential branching fractions and isospin asymmetries of $B \to K^{(*)}\mu^{+}\mu^{-}$ decays

The isospin asymmetries of $B \to K\mu^+\mu^-$ and $B \to K^{*}\mu^+\mu^-$ decays and the partial branching fractions of the $B^0 \to K^0\mu^+\mu^-$, $B^+ \to K^+\mu^+\mu^-$ and $B^+ \to K^{*+}\mu^+\mu^-$ decays are measured as functions of the dimuon mass squared, $q^2$. The data used correspond to an integrated luminosity of 3$~$fb$^{-1}$ from proton-proton collisions collected with the LHCb detector at centre-of-mass energies of 7$\,$TeV and 8$\,$TeV in 2011 and 2012, respectively. The isospin asymmetries are both consistent with the Standard Model expectations. The three measured branching fractions, while individually consistent, all favour lower values than their respective Standard Model predictions.

==> dataset.tex <==



